Level Set Teleportation: An Optimization Perspective

We study level set teleportation, an optimization routine which tries to accelerate gradient descent (GD) by maximizing the gradient norm over a level set of the objective. While teleportation intuitively speeds-up GD via bigger steps, current work lacks convergence theory for convex functions, guarantees for solving the teleportation operator, and even clear empirical evidence showing this acceleration. We resolve these open questions. For convex functions satisfying Hessian stability, we prove that GD with teleportation obtains a combined sub-linear/linear convergence rate which is strictly faster than GD when the optimality gap is small. This is in sharp contrast to the standard (strongly) convex setting, where teleportation neither improves nor worsens convergence. To evaluate teleportation in practice, we develop a projected-gradient method requiring only Hessian-vector products. We use this to show that gradient methods with access to a teleportation oracle out-perform their standard versions on a variety of problems. We also find that GD with teleportation is faster than truncated Newton methods, particularly for non-convex optimization.

==> appendices/algorithm.tex <==
Now we briefly discuss how to terminate our algorithm.
Suppose that \( \bar x \) is a local maximum of \cref{eq:sublevel-teleport}.
If the linear independence constraint qualification (LICQ) holds, 
then \( \bar x \) must satisfy the KKT conditions for some \( \lambda > 0 \)
\citep{bertsekas1997nonlinear},
\begin{align}\label{eq:kkt-conditions}
    \nabla^2 f(\xk) \grad(\xk) / \norm{\grad(\xk)} + \lambda \grad(\xk)
    &= 0,\\ 
    f(\xk) \leq f(\wk) \quad \text{and} \quad \lambda (f(\xk) - f(\wk)) &= 0. \nonumber
\end{align}
That is, \( \nabla^2 f(\xk) \grad(\xk) \propto \grad(\xk) \) and the 
sub-level set constraint is satisfied.
The teleportation problem satisfies LICQ unless \( \grad(\bar x) =
0 \); 
in this case, stationarity at \( \bar x \) implies stationarity over all of \(
\calS_k \) and teleporting is not interesting.
Thus, we assume LICQ holds and combine termination based on the KKT conditions
with line-search to give a complete solver in \cref{alg:teleport}.


==> macros/tags <==
!_TAG_FILE_FORMAT	2	/extended format; --format=1 will not append ;" to lines/
!_TAG_FILE_SORTED	1	/0=unsorted, 1=sorted, 2=foldcase/
!_TAG_OUTPUT_FILESEP	slash	/slash or backslash/
!_TAG_OUTPUT_MODE	u-ctags	/u-ctags or e-ctags/
!_TAG_PATTERN_LENGTH_LIMIT	96	/0 for no limit/
!_TAG_PROGRAM_AUTHOR	Universal Ctags Team	//
!_TAG_PROGRAM_NAME	Universal Ctags	/Derived from Exuberant Ctags/
!_TAG_PROGRAM_URL	https://ctags.io/	/official site/
!_TAG_PROGRAM_VERSION	0.0.0	/62f0144/
\\Dim	math.tex	/^\\newcommand{\\Dim}{\\text{Dim}}$/;"	C
\\Lk	math.tex	/^\\newcommand{\\Lk}{L_{\\zk}}$/;"	C
\\Lmax	math.tex	/^\\newcommand{\\Lmax}{L_{\\text{max}}}$/;"	C
\\Lmin	math.tex	/^\\newcommand{\\Lmin}{L_{\\text{min}}}$/;"	C
\\Null	math.tex	/^\\newcommand{\\Null}{\\text{Null}}$/;"	C
\\Var	math.tex	/^\\newcommand{\\Var}[1]{\\textbf{Var}\\sbr{#1}}$/;"	C
\\Z	math.tex	/^\\newcommand{\\Z}{Z}$/;"	C
\\abr	math.tex	/^\\newcommand{\\abr}[1]{\\left\\langle#1\\right\\rangle}$/;"	C
\\abs	math.tex	/^\\newcommand{\\abs}[1]{\\left\\vert #1\\right\\vert}$/;"	C
\\addnumber	math.tex	/^\\newcommand{\\addnumber}{\\addtocounter{equation}{1}\\tag{\\theequation}}$/;"	C
\\alphak	math.tex	/^\\newcommand{\\alphak}{\\alpha_{k}}$/;"	C
\\alphakk	math.tex	/^\\newcommand{\\alphakk}{\\alpha_{k+1}}$/;"	C
\\argdot	math.tex	/^\\newcommand{\\argdot}{{\\,\\vcenter{\\hbox{\\tiny$\\bullet$}}\\,}} %generic argument dot$/;"	C
\\as	math.tex	/^\\newcommand{\\as}[1]{\\stackrel{\\text{\\rm\\tiny a.s.}}{#1}}$/;"	C
\\aside	paragraph.tex	/^\\newcommand{\\aside}[1]{(\\textcolor{red}{\\textbf{Aside}: #1})}$/;"	C
\\betak	math.tex	/^\\newcommand{\\betak}{\\beta_{k}}$/;"	C
\\betakk	math.tex	/^\\newcommand{\\betakk}{\\beta_{k+1}}$/;"	C
\\biggmid	math.tex	/^\\newcommand{\\biggmid}{\\bigg \\vert }$/;"	C
\\cbr	math.tex	/^\\newcommand{\\cbr}[1]{\\left\\{#1\\right\\}}$/;"	C
\\col	math.tex	/^\\newcommand{\\col}{\\text{Col}}$/;"	C
\\dist	math.tex	/^\\newcommand{\\dist}[1]{\\stackrel{\\text{\\rm\\tiny dist}}{#1}}$/;"	C
\\dom	math.tex	/^\\newcommand{\\dom}{\\text{Dom}}$/;"	C
\\eR	math.tex	/^\\newcommand{\\eR}{\\bar{\\mathbb{R}}}$/;"	C
\\equas	math.tex	/^\\newcommand{\\equas}{\\stackrel{\\text{\\rm\\tiny a.s.}}{=}}$/;"	C
\\equdist	math.tex	/^\\newcommand{\\equdist}{\\stackrel{\\text{\\rm\\tiny dist}}{=}}$/;"	C
\\etak	math.tex	/^\\newcommand{\\etak}{\\eta_k}$/;"	C
\\etakk	math.tex	/^\\newcommand{\\etakk}{\\eta_{k+1}}$/;"	C
\\etamax	math.tex	/^\\newcommand{\\etamax}{\\eta_{\\text{max}}}$/;"	C
\\etamin	math.tex	/^\\newcommand{\\etamin}{\\eta_{\\text{min}}}$/;"	C
\\f	math.tex	/^\\newcommand{\\f}{f}$/;"	C
\\fj	math.tex	/^\\newcommand{\\fj}{f_i}$/;"	C
\\fk	math.tex	/^\\newcommand{\\fk}{f_{i_k}}$/;"	C
\\fkk	math.tex	/^\\newcommand{\\fkk}{f_{i_{(k+1)}}}$/;"	C
\\fopt	math.tex	/^\\newcommand{\\fopt}{f^*}$/;"	C
\\grad	math.tex	/^\\newcommand{\\grad}{\\nabla f}$/;"	C
\\gradk	math.tex	/^\\newcommand{\\gradk}{\\nabla f_{i_k}}$/;"	C
\\gradkk	math.tex	/^\\newcommand{\\gradkk}{\\nabla f_{i_{(k+1)}}}$/;"	C
\\halved	math.tex	/^\\newcommand{\\halved}[1]{\\frac{#1}{2}}$/;"	C
\\ind	math.tex	/^\\newcommand{\\ind}[0]{\\perp \\!\\!\\! \\perp }$/;"	C
\\into	math.tex	/^\\newcommand{\\into}{\\rightarrow}$/;"	C
\\inv	math.tex	/^\\newcommand{\\inv}[1]{\\frac{1}{#1}}$/;"	C
\\iter	math.tex	/^\\newcommand{\\iter}{k}$/;"	C
\\mumax	math.tex	/^\\newcommand{\\mumax}{\\mu_{\\text{max}}}$/;"	C
\\mumin	math.tex	/^\\newcommand{\\mumin}{\\mu_{\\text{min}}}$/;"	C
\\oracle	math.tex	/^\\newcommand{\\oracle}{\\mbox{\\( \\calO \\)}}$/;"	C
\\rbr	math.tex	/^\\newcommand{\\rbr}[1]{\\left(#1\\right)}$/;"	C
\\row	math.tex	/^\\newcommand{\\row}{\\text{Row}}$/;"	C
\\sbr	math.tex	/^\\newcommand{\\sbr}[1]{\\left[#1\\right]}$/;"	C
\\seq	math.tex	/^\\newcommand{\\seq}[1]{\\rbr{#1}}$/;"	C
\\sgc	math.tex	/^\\newcommand{\\sgc}{\\rho}$/;"	C
\\tetak	math.tex	/^\\newcommand{\\tetak}{{\\tilde{\\eta}}_{k}}$/;"	C
\\vk	math.tex	/^\\newcommand{\\vk}{v_k}$/;"	C
\\vkk	math.tex	/^\\newcommand{\\vkk}{v_{k+1}}$/;"	C
\\vspan	math.tex	/^\\newcommand{\\vspan}{\\text{Span}}$/;"	C
\\w	math.tex	/^\\newcommand{\\w}{w}$/;"	C
\\wbar	math.tex	/^\\newcommand{\\wbar}{\\bar{w}}$/;"	C
\\wgc	math.tex	/^\\newcommand{\\wgc}{\\alpha}$/;"	C
\\wk	math.tex	/^\\newcommand{\\wk}{w_k}$/;"	C
\\wkk	math.tex	/^\\newcommand{\\wkk}{w_{k+1}}$/;"	C
\\wopt	math.tex	/^\\newcommand{\\wopt}{w^*}$/;"	C
\\x	math.tex	/^\\newcommand{\\x}{x}$/;"	C
\\xbar	math.tex	/^\\newcommand{\\xbar}{\\xbar{w}}$/;"	C
\\xk	math.tex	/^\\newcommand{\\xk}{x_k}$/;"	C
\\xkk	math.tex	/^\\newcommand{\\xkk}{x_{k+1}}$/;"	C
\\xkplus	math.tex	/^\\newcommand{\\xkplus}{x_k^+}$/;"	C
\\xopt	math.tex	/^\\newcommand{\\xopt}{x^*}$/;"	C
\\y	math.tex	/^\\newcommand{\\y}{y}$/;"	C
\\yk	math.tex	/^\\newcommand{\\yk}{y_k}$/;"	C
\\ykk	math.tex	/^\\newcommand{\\ykk}{y_{k+1}}$/;"	C
\\z	math.tex	/^\\newcommand{\\z}{z}$/;"	C
\\zk	math.tex	/^\\newcommand{\\zk}{z_{k}}$/;"	C
\\zkk	math.tex	/^\\newcommand{\\zkk}{z_{k+1}}$/;"	C
macros	README.md	/^# macros$/;"	c

